Homa: A Receiver-Driven Low-Latency Transport Protocol Using Network Priorities (Complete Version)

Homa is a new transport protocol for datacenter networks. It provides exceptionally low latency, especially for workloads with a high volume of very short messages, and it also supports large messages and high network utilization. Homa uses in-network priority queues to ensure low latency for short messages; priority allocation is managed dynamically by each receiver and integrated with a receiver-driven flow control mechanism. Homa also uses controlled overcommitment of receiver downlinks to ensure efficient bandwidth utilization at high load. Our implementation of Homa delivers 99th percentile round-trip times less than 15{\mu}s for short messages on a 10 Gbps network running at 80% load. These latencies are almost 100x lower than the best published measurements of an implementation. In simulations, Homa's latency is roughly equal to pFabric and significantly better than pHost, PIAS, and NDP for almost all message sizes and workloads. Homa can also sustain higher network loads than pFabric, pHost, or PIAS.

==> fig-overcommit.tex <==
\begin{figure}
\begin{center}
\includegraphics[scale=0.40]{overcommit2}
\caption{Overcommitment with preemption. Both S1 and S2 have
long messages for R1. (a) R1 issues
grants for both messages, using P1 for \emph{m2} (since it is shorter)
and P0 for \emph{m1}. Packets for \emph{m2} are delivered to R1;
RTTbytes of packets for \emph{m1} are buffered in
the TOR. (b) Before completing \emph{m2}, a new shorter message \emph{m3}
is created at S2 for R2. S2 preempts \emph{m2} and begins transmitting \emph{m3}
to R2. Buffered packets for \emph{m1} can then flow to
R1 and the P0 queue drains. As R1 receives packets of \emph{m1}, it
issues new grants; packets from these new grants begin arriving at
the TOR just as the P0 queue becomes empty.  When S2 finishes
sending \emph{m3}, it resumes sending \emph{m2}. The packets for \emph{m2} take
precedence over those for \emph{m1}, so buffering will build up again
as in (a).
}
\label{fig:overcommit}
\end{center}
\end{figure}


==> fig-schedPriorities.tex <==
\begin{figure}
\begin{center}
\includegraphics[scale=0.6]{schedPriorities}
\caption{Allocation of scheduled priorities (3 priorities are available
for scheduled packets): (a) two messages are
currently being granted (M2 is shorter, so it has higher priority);
(b) new message M3 arrives
(it is shorter than M2); (c) new message M4 arrives (it is shorter
than M3).
}
\label{fig:schedPriorities}
\end{center}
\end{figure}


==> fig-slowdownVsPrioBalance.tex <==
\begin{figure}
\begin{center}
\includegraphics[scale=0.14]{slowdownVsSchedUnschedPrioCutoff}
\caption{The impact on slowdown of the balance between unscheduled and
scheduled priority levels. Each curve uses 8 total priority levels,
but with a different tradeoff between unscheduled and scheduled levels.
All measurements used workload W2 at 80\% network load.  
}
\label{fig:slowdownVsPrioBalance}
\end{center}
\end{figure}


==> fig-slowdownVsPrioLevels.tex <==
\begin{figure}
\begin{center}
\includegraphics[scale=0.14]{slowdownVsPrioLevels}
\caption{Impact of the total number of priority levels on
the W3 workload (80\% network load).  
}
\label{fig:slowdownVsPrioLevels}
\end{center}
\end{figure}


==> fig-spectrumTail50.tex <==
\begin{figure}
\begin{center}
\includegraphics[scale=0.12]{spectrumTail50_noOracle}
\caption{99th-percentile slowdown as a function of message size,
for different protocols and workloads, at a network load of
50\%. Distance on the x-axis is linear in total number of messages
(each tick corresponds to 10\% of all messages). 
}
\label{fig:spectrumTail50}
\end{center}
\end{figure}


==> fig-spectrumTail80.tex <==
\begin{figure}
\begin{center}
\includegraphics[scale=0.11]{spectrumTail80_noOracle}
\caption{99th-percentile slowdown as a function of message size,
for different protocols and workloads, at a network load of
80\%. Distance on the x-axis is linear in total number of messages
(each tick corresponds to 10\% of all messages). The minimum
one-way time for a small message (slowdown is 1.0) is 2.3 $\upmu$s.
NDP was measured only for W5; it used a network load of 70\%.
}
\label{fig:spectrumTail80}
\vspace{\figSqueeze{}}
\end{center}
\end{figure}

